ICAR: Image-based Complementary Auto Reasoning

Scene-aware Complementary Item Retrieval (CIR) is a challenging task which requires to generate a set of compatible items across domains. Due to the subjectivity, it is difficult to set up a rigorous standard for both data collection and learning objectives. To address this challenging task, we propose a visual compatibility concept, composed of similarity (resembling in color, geometry, texture, and etc.) and complementarity (different items like table vs chair completing a group). Based on this notion, we propose a compatibility learning framework, a category-aware Flexible Bidirectional Transformer (FBT), for visual "scene-based set compatibility reasoning" with the cross-domain visual similarity input and auto-regressive complementary item generation. We introduce a "Flexible Bidirectional Transformer (FBT)" consisting of an encoder with flexible masking, a category prediction arm, and an auto-regressive visual embedding prediction arm. And the inputs for FBT are cross-domain visual similarity invariant embeddings, making this framework quite generalizable. Furthermore, our proposed FBT model learns the inter-object compatibility from a large set of scene images in a self-supervised way. Compared with the SOTA methods, this approach achieves up to 5.3% and 9.6% in FITB score and 22.3% and 31.8% SFID improvement on fashion and furniture, respectively.

==> figures/fashion_more.tex <==
\begin{figure*}[th]
\centering
\includegraphics[width=1.0\textwidth]{figs/fashion_more.pdf}
\caption{\textbf{More Visualization for Fashion.}
}
\label{fig:fashion_more}
\end{figure*}

==> figures/taser.tex <==
\begin{figure*}[t]
%\vspace{-3mm}
\centering
    \includegraphics[width=\textwidth]{figs/teaser.pdf}
    \caption{\textbf{Imaged-based Complementary Auto Reasoning.} 
    We present a new two-stage self-supervised model for scene-aware, visually compatible cross-domain object retrieval task. In this example, given an inspirational home scene image (sampled from STL-home\cite{kang2019complete} column 1, 3, 5) with a pool of objects (3D-FRONT\cite{fu20213d}) from an unseen domain, our model auto-regressively retrieves a set of stylistically compatible items (column 2, 4, 6).
    %We are also one of the first to demonstrate the capability of generalizing to unseen domain for the scene-aware cross-domain CIR task.
    We build our model based on the intuition of dividing the task into: cross-domain retrieval and complementary reasoning.
    In the first stage, we apply a CNN-based model to learn the visual similarity between the two domains. 
    Then, in the second stage, we propose a category-aware {\em Flexible Bidirectional Transformer} model to automatically reason about the item visual compatibility.
    %\JL{add more details. e.g., using what new techniques?} 
    %Our model learns to reason about the visual compatibility from a large set of scene images. 
    %Note: the 3D placement and orientation in this example are pre-generated. (\JL{I don't think this matters and should be added in the teaser's caption}).
    }
    \label{fig:teaser}
    \vspace{6mm}
\end{figure*}

==> sections/cltr.tex <==
% Complementary Transformer (CLTR) is a framework to perform the task of complementary products recommendation. CLTR learns to generate sets of complementary products without the need of annotations by professionals. To achieve this, CLTR learns the complementarity directly through lifestyle images using a Transformer architecture. The model starts with a scene image of a room. Products are detected and passed along with the query image (i.e., global context) to the Transformer to generate a complementary item recommendation set. The algorithm includes four components: a CNN-based image encoder that computes the image embedding, an encoder-decoder Transformer model to produce representations of complementarity items, a two-headed feed-forward network to predict category labels and embeddings of the recommended items, and a retrieval module to generate the final complementary recommendations. Comparing to existing work, the algorithm requires no expert annotations for training. Also, the pipeline removes the burden of pair-to-set generation and hand-designed components. Additionally, the model directly infers the category information of the output set so no category information are needed as input. Thus, the system can be easily scaled to large datasets and generalized to other domains.

==> tables/category.tex <==
\begin{table}
\centering
\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{c c c }
\toprule
Method & FITB \uparrow & Condition   \\
\midrule 
ICAR w/o Cate. Embedding & / & Predict the target cate. \\
ICAR w Cate. Embedding & 83.9 & Predict the target cate. \\
ICAR w/o Cate. Embedding & 86.2 & Given the target cate. \\
ICAR w Cate. Embedding & 87.1 & Given the target cate. \\
\bottomrule 
\end{tabular}
}
\caption{{\bf Category Embedding Ablation Study.} We demonstrate that our category embedding improves the recommendation performance.}
\label{tab:category}
\end{table}

==> tables/s2s.tex <==
\begin{table}[!h]
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{c c c }
\toprule
Method & FITB \uparrow & Negative num   \\
\midrule 
IBR \cite{mcauley2015image} & 56.5 & 1 \\
Siamese Nets  \cite{veit2015learning} & 63.0  & 1 \\
BPR-DAE \cite{song2017neurostylist} & 59.3 & 1 \\
Complete the Look \cite{kang2019complete}  & 63.1 & 1 \\
CLTR (see Sec. 1 Supp)   & 67.2 & 1 \\
\midrule 
\textbf{ICAR (Ours)}  & \textbf{71.4} & 1 \\
\bottomrule 
\end{tabular}
}
\caption{Results on Street2Shop. We demonstrate that our approach can improve the FITB accuracy by 8.3\%.}
\label{tab:s2s}
\end{table}

==> tables/style_home_sfid.tex <==
\begin{table}
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{c c c}
\toprule
Method & SFID \downarrow & Set Number   \\
\midrule 
bbox GT VS bbox Neg & $75.2$ & 5  \\
non-bbox GT VS non-bbox Neg & $49.0$ & 5\\
CLTR (see Sec. 1 Supp)  & $48.0$  & 5\\
\midrule 
\textbf{ICAR (Ours)}  & \textbf{36.8} & 5\\
\bottomrule 
\end{tabular}
}
\caption{Results on DeepRooms using SFID.  Our approach improved the SFID accuracy by {\bf 11.6\%}.}
\label{tab:style_home_sfid}
\end{table}
